PACSET (Packed Serialized Trees): Reducing Inference Latency for Tree Ensemble Deployment

We present methods to serialize and deserialize tree ensembles that optimize inference latency when models are not already loaded into memory. This arises whenever models are larger than memory, but also systematically when models are deployed on low-resource devices, such as in the Internet of Things, or run as Web micro-services where resources are allocated on demand. Our packed serialized trees (PACSET) encode reference locality in the layout of a tree ensemble using principles from external memory algorithms. The layout interleaves correlated nodes across multiple trees, uses leaf cardinality to collocate the nodes on the most popular paths and is optimized for the I/O blocksize. The result is that each I/O yields a higher fraction of useful data, leading to a 2-6 times reduction in classification latency for interactive workloads.

==> mlsys2020style/tikz_figures/blockinference.tex <==
%\usetikzlibrary{shapes.geometric }
 
\tikzset{    database/.style={
      cylinder,
      text width=11em,
      cylinder uses custom fill,
      cylinder body fill=yellow!50,
      cylinder end fill=yellow!50,
      shape border rotate=90,
      aspect=0.3,
      draw
    } }

% Define block styles
\tikzstyle{decision} = [diamond, draw,   fill=blue!20, 
    text width=4em, text badly centered,  node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw,    fill=blue!20, 
    text width=4em, text centered,  minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw,  circle,fill=red!20, node distance=5cm,  
    minimum height=2em, text width=4em]
    
         \begin{tikzpicture}[node distance = 12cm,auto]
            % Place nodes
            \node [database] (init) { 1. Packed PACSET Model\\2. Test Data};
            %\node[database, below of=init](data) {Inference Data};
            %\node [block, right of=read] (infer) {Perform Inference};
            \node[cloud, right of=init](results){Results};
            % Draw edges
            \path [line] (init) -- (results);
            %\path [line] (data) -| (results);
            %\path [line] (infer) -- (results);
        \end{tikzpicture}
 

==> mlsys2020style/tikz_figures/blockpack.tex <==
\usetikzlibrary{shapes.geometric}
 

\tikzset{    database/.style={
      cylinder,
      text width=4em,
      cylinder uses custom fill,
      cylinder body fill=yellow!50,
      cylinder end fill=yellow!50,
      shape border rotate=90,
      aspect=0.3,
      draw
    } }

% Define block styles
\tikzstyle{decision} = [diamond, draw,   fill=blue!20, 
    text width=4em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=4em, text centered,   minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, circle,fill=red!20, node distance=3cm,  
    minimum height=2em, text width=4em]
    
\begin{tikzpicture}[node distance = 3cm,auto]
            % Place nodes
            \node [database] (init) {Trained JSON Model};
            % \node [block, right of=init] (read) {Read Model};
            % \node [block, right of=read] (pack) {Pack Model};
            \node[cloud, right of=init](packedmodel){Pack Model};
            % \node [block, right of=packedmodel] (store) {Store Model};
            \node [database, right of=packedmodel] (storedmodel) {Packed PACSET Model};
            % Draw edges
            %\path [line] (init) -- (read);
            %\path [line] (read) -- (pack);
             \path [line] (init) -- (packedmodel);
            % \path [line] (packedmodel) -- (store);
             \path [line] (packedmodel) -- (storedmodel);
\end{tikzpicture}
